Fact-and-Reflection (FaR) Improves Confidence Calibration of Large Language Models

For a LLM to be trustworthy, its confidence level should be well-calibrated with its actual performance. While it is now common sense that LLM performances are greatly impacted by prompts, the confidence calibration in prompting LLMs has yet to be thoroughly explored. In this paper, we explore how different prompting strategies influence LLM confidence calibration and how it could be improved. We conduct extensive experiments on six prompting methods in the question-answering context and we observe that, while these methods help improve the expected LLM calibration, they also trigger LLMs to be over-confident when responding to some instances. Inspired by human cognition, we propose Fact-and-Reflection (FaR) prompting, which improves the LLM calibration in two steps. First, FaR elicits the known "facts" that are relevant to the input prompt from the LLM. And then it asks the model to "reflect" over them to generate the final answer. Experiments show that FaR prompting achieves significantly better calibration; it lowers the Expected Calibration Error by 23.5% on our multi-purpose QA tasks. Notably, FaR prompting even elicits the capability of verbally expressing concerns in less confident scenarios, which helps trigger retrieval augmentation for solving these harder instances.

==> ToT_example.tex <==
Bob is in the living room.
He walks to the kitchen, carrying a cup.
He puts a ball in the cup and carries the cup to the bedroom.
He turns the cup upside down, then walks to the garden.
He puts the cup down in the garden, then walks to the garage.
Where is the ball?


=====



Expert 1: The ball is in the living room.

Expert 2: The ball is in the kitchen.

Expert 3: The ball is in the bedroom.

Expert 1: Bob carries the cup to the bedroom, so the ball must be in the cup.

Expert 2: Oh, I see my mistake. Yes, the ball is in the cup.

Expert 3: Agreed, the ball is in the cup in the bedroom.

Expert 1: Next, Bob turns the cup upside down in the bedroom.

Expert 2: After that, Bob walks to the garden and puts the cup down.

Expert 3: Therefore, the ball must have fallen out of the cup when Bob turned it upside down in the bedroom. So, the ball is in the bedroom, not in the cup anymore.

Expert 1: Oh, you're right. I made a mistake. The ball is in the bedroom, not in the cup.

Expert 2: Agreed, the ball is in the bedroom.

Expert 3: Bob then walks to the garage, so the ball remains in the bedroom. It is not in the garden or the garage.

Expert 1: Absolutely, the ball is still in the bedroom.

Expert 2: Yes, the ball hasn't moved from the bedroom.

Expert 3: Therefore, the ball is in the bedroom, not in the garden or the garage.

All three experts agree that the ball is in the bedroom.
